Matrix-product-state GPLHR for non-Hermitian many-body eigenproblems

Computing multiple eigenstates of non-Hermitian many-body operators plays an important role in investigating excitation spectra, spectral properties, and relaxation dynamics in interacting and open quantum systems. However, this task is challenging because the eigenvectors are generally nonorthogonal and the Hilbert space dimension grows exponentially with system size. Here, we formulate the generalized preconditioned locally harmonic residual (GPLHR) method in a matrix product state (MPS) framework to efficiently compute multiple targeted right eigenstates whose eigenvalues lie near a specified shift in the complex plane. Successive randomized compression (SRC) is employed to accelerate operator applications. We test the method on transcorrelated and complex Hubbard chains, an interacting non-Hermitian Su-Schrieffer-Heeger (SSH) chain, and a Liouvillian model. The results demonstrate that GPLHR combined with MPS provides an efficient and accurate approach for computing multiple eigenstates of non-Hermitian many-body operators.

==> authors.tex <==
\makeatletter

\DeclareRobustCommand{\equalcontrib}{%
  \@booleantrue\equalcontrib@sw
}

\def\equalcontribtext{%
  These authors contributed equally to this work.%
}

\def\doauthor#1#2#3{%
  \@booleanfalse\equalcontrib@sw
  \ignorespaces#1\unskip\@listcomma
  \begingroup
    #3%
  \equalcontrib@sw{%
    \endgroup{\comma@space}{}%
    \frontmatter@footnote{\equalcontribtext}%
    \@if@empty{#2}{}{%
      \comma@space\frontmatter@footnote{#2}%
    }%
  }{%
    \@if@empty{#2}%
      {\endgroup{}{}}%
      {\endgroup{\comma@space}{}%
       \frontmatter@footnote{#2}}%
  }%
  \space\@listand
}

\makeatother

\author{Xingyao Wu\,\orcidlink{0009-0009-7762-9038}}
\affiliation{Technical University of Munich, Department of Physics,
85748 Garching, Germany}
\affiliation{Technical University of Munich, CIT, Department of Computer Science, Boltzmannstra{\ss}e 3, 85748 Garching, Germany}



\author{Zhangyu Yang\,\orcidlink{0009-0009-1589-7985}}
\email{zhangyuyang@link.cuhk.edu.cn}
\affiliation{School of Science and Engineering,
The Chinese University of Hong Kong (Shenzhen),
Longgang, Shenzhen 518172, Guangdong, P.R. China}

\author{Yanbin Chen\,\orcidlink{0000-0002-1123-1432}}
\affiliation{Technical University of Munich, CIT, Department of Computer Science, Boltzmannstra{\ss}e 3, 85748 Garching, Germany}

\author{Yu Wang\,\orcidlink{0009-0004-3972-4388}}
\email{ywang96@sdu.edu.cn}
%\email{18yu.wang@tum.de}
\affiliation{Technical University of Munich, CIT, Department of Computer Science, Boltzmannstra{\ss}e 3, 85748 Garching, Germany}
\affiliation{Key Laboratory for Colloid and Interface
Chemistry, Ministry of Education, School of Chemistry and
Chemical Engineering, Shandong University, Qingdao
266237, China}


\author{Feng Chen\,\orcidlink{0000-0001-8196-030X}}
\email{fchen@cuhk.edu.cn}
\affiliation{School of Science and Engineering,
The Chinese University of Hong Kong (Shenzhen),
Longgang, Shenzhen 518172, Guangdong, P.R. China}
